Illuminating the Dark Sector: Searching for new interactions between dark matter and dark energy

The current standard model of cosmology - the {\ensuremath{\Lambda}}CDM model - is appropriately named after its controversial foreign ingredients: a cosmological constant ({\ensuremath{\Lambda}}) that accounts for the recent accelerated expansion of the Universe and cold dark matter needed to explain the formation and dynamics of large scale structures. Together, these form the dark sector, whose nature remains a mystery. After 25 years of withstanding confirmation and support for the {\ensuremath{\Lambda}}CDM model, enough to bypass some of its unclear theoretical issues, this paradigm is facing its biggest crisis yet. The rapid advent of technology has brought cosmology to an unprecedented observational era, with increased technical precision and the emergence of independent measures, including probes of phenomena that were thought impossible to detect or even exist, such as the gravitational ripples that propagate in the spacetime. However, such precision has unveiled cracks in the porcelain of {\ensuremath{\Lambda}}CDM, with pieces that seem glued together and difficult to reconcile. Particularly worrying is the apparent lack of compatibility between measurements of the Universe's present expansion rate based on local measurements and those based on phenomena that occurred far in the early Universe and that can only be translated into present quantities through physical propagation under a cosmological model. In this dissertation, we delve into extensions to the standard model that consider alternatives to the mysterious nature of the dark sector and any possible new interactions therein. We analyse these alternative models, hoping to identify measurable observational signatures of extra degrees of freedom in the dark sector.

==> Chapters/Conventions.tex <==
%Main in MyThesis.tex

\chapter*{Conventions and Units}
\chaptermark{Conventions and Units}
\addcontentsline{toc}{fmchapter}{Conventions and Units}
\setcounter{equation}{0}
\setcounter{figure}{0}

\subsubsection{Units}

Unless stated otherwise, in this dissertation I will always adopt natural units in which the speed of light, Planck's constant and Boltzmann's constant are unity, $c=\hbar = k_B = 1$. This translates into an equivalence of units for energy, mass and momentum as an inverse unit of length and time: 
%
\begin{equation}
    \text{[Energy]} = \text{[Mass]} = \text{[Temperature]} = \text{[Length]}^{-1} = \text{[Time]}^{-1} \mathperiod
    \end{equation}
%
Different units may be adopted for numerical purposes and these are described in \cref{sec:appa}.

Some useful conversion factors for these units are listed below:

Some useful fundamental constants are listed below:

\subsubsection{Background FLRW Metric}

\subsection{Perturbed FLRW Metric}


Throughout this manuscript we denote derivatives with respect to physical time $t$ by an upper dot and derivatives with respect to conformal time $\tau$ by a prime,
%
\begin{align}
t = \text{cosmic time}\ \ &\Longrightarrow \ \ \frac{\dd X}{\dd t} \equiv \dot{X} \mathcomma \\
\tau = \text{conformal time}\ \ &\Longrightarrow \ \ \frac{\dd X}{\dd \tau} \equiv X' \mathperiod
\end{align}

Spatial 3-vectors are denoted in bold face, such as $\vec{x}$ and four-dimensional spacetime vectors are denoted in terms of their components as $x = (x^{\mu})$.

We adopt the convention for the signature of the metric as $(-,+,+,+)$.

Fourier transforms are defined as
%
\be
f (\vec{k}) = \int \dd^3 x\, f(\vec{x})\, e^{i \vec{k} \cdot \vec{x}} \mathcomma
\ee
%
such that the inverse is given by
%
\be 
f(\vec{x}) = \frac{1}{\left(2 \pi\right)^3} \int \dd^3 k\, f(\vec{k})\, e^{-i \vec{k} \cdot \vec{x}} \mathperiod
\ee
%
This allows us to define the spectrum $P_f (k)$ of any statistically homogeneous and isotropic random variable $f$
%
\be
\langle f (\vec{k}) f^* (\vec{k'})  \rangle = \left( 2 \pi \right)^3 \delta \left( \vec{k} - \vec{k'} \right) P_f (k) \mathperiod
\ee
%
Being isotropic, $P_f (k)$ can be described simply in terms of the modulus $k = | \vec{k} |$. When $f$ is a Gaussian it is implied that the $\vec{k}$ modes are uncorrelated through the Dirac delta function.

\subsubsection{Primordial Power Spectrum}

==> Chapters/Declaration.tex <==
\chapter*{Declaration}
\chaptermark{Declaration}
\addcontentsline{toc}{fmchapter}{Declaration}

I hereby declare that except where specific reference is made to the work of others, the contents of this thesis are original and have not been submitted in whole or in part for the consideration for any other degree or qualification in this or any other University. This thesis has been composed by myself and contains nothing which is the outcome of work done in collaboration with others, except when specified.


Before moving on I would just like to acknowledge the relevant software, numerical tools and observational data sets used. Wherever the numerical evolution of a cosmological scenario is mentioned this was conducted following our own modified version of the Einstein-Boltzmann solver \texttt{CLASS} \cite{lesgourgues2011cosmic,Blas_2011,lesgourgues2011cosmic2}. Moreover, references to comparison of a given theory to data always imply the use of \texttt{MontePython} \cite{Audren_2013,Brinckmann:2018cvx}, a Python Monte Carlo Markov Chain sampling code for parameter inference in cosmology, that can be interfaced with \texttt{CLASS} and modified according to the particular setting. The results reported in the tables and figures are produced with the aid of the \texttt{GetDist} Python package \cite{Lewis:2019xzd} and the statistical significance when compared with the benchmark $\Lambda$CDM setting is assessed through the \texttt{MCEvidence} package \cite{2017arXiv170403472H}. To perform the simulations we used to the HPC system facilities of the University of Sheffield, in particular \texttt{Sharc} and \texttt{Bessemer}.
Finally, unless otherwise stated, the data sets used for the study of observational constraints are particular combinations of the CMB {\it Planck} 2018 \cite{Planck:2019nip} data, a compilation of BAO distance and expansion rate measurements from the Sloan Digital Sky Survey (SDSS) DR7 Main Galaxy Sample \cite{Ross:2014qpa}, SDSS DR12 consensus release \cite{BOSS:2016hvq} and the 6dF Galaxy Survey \cite{Beutler:2011hx}, and distance moduli measurements of type Ia Supernova (SN) data from the Pantheon collaboration \cite{Scolnic:2017caz}.

==> Chapters/List_Papers.tex <==
%Main in MyThesis.tex

\section*{List of Papers}


% Add entry in the table of contents as section
%\addcontentsline{toc}{section}{\acknowledgments}

Include comment on my contribution to each paper?

The following papers are included in the thesis. They are referred to by their Roman numerals in the text.

The following are additional papers I worked on during my PhD but which did not fit within the storyline of this thesis and are not included. They are quoted as ordinary references in the main text where appropriate.

==> Chapters/Notation.tex <==
\chapter*{Notation}
\chaptermark{Notation}
\addcontentsline{toc}{fmchapter}{Notation}

